Safety and Liveness Guarantees through Reach-Avoid Reinforcement Learning

Reach-avoid optimal control problems, in which the system must reach certain goal conditions while staying clear of unacceptable failure modes, are central to safety and liveness assurance for autonomous robotic systems, but their exact solutions are intractable for complex dynamics and environments. Recent successes in reinforcement learning methods to approximately solve optimal control problems with performance objectives make their application to certification problems attractive; however, the Lagrange-type objective used in reinforcement learning is not suitable to encode temporal logic requirements. Recent work has shown promise in extending the reinforcement learning machinery to safety-type problems, whose objective is not a sum, but a minimum (or maximum) over time. In this work, we generalize the reinforcement learning formulation to handle all optimal control problems in the reach-avoid category. We derive a time-discounted reach-avoid Bellman backup with contraction mapping properties and prove that the resulting reach-avoid Q-learning algorithm converges under analogous conditions to the traditional Lagrange-type problem, yielding an arbitrarily tight conservative approximation to the reach-avoid set. We further demonstrate the use of this formulation with deep reinforcement learning methods, retaining zero-violation guarantees by treating the approximate solutions as untrusted oracles in a model-predictive supervisory control framework. We evaluate our proposed framework on a range of nonlinear systems, validating the results against analytic and numerical solutions, and through Monte Carlo simulation in previously intractable problems. Our results open the door to a range of learning-based methods for safe-and-live autonomous behavior, with applications across robotics and automation. See https://github.com/SafeRoboticsLab/safety_rl for code and supplementary material.

==> appendices/shielding.tex <==
\section{Learning-Based Reach-Avoid Guarantees during Learning and Exploration}
\begin{itemize}
    \item How do we turn this into actual guarantees?
    \item Safe Learning and ``Shielding".
    \item Learned Q-value as an untrusted oracle: check with forward sim.
    \item \textbf{Theorem}: Suppose $\tilde\policy$, simulated forward from $\state$, is predicted to reach $\target$ while avoiding $\failure$. Then, the following least-restrictive ``shielding" law is guaranteed to recursively preserve safety and liveness:
    \begin{equation}
    \policy_{\text{shield}}(\state)=
        \begin{cases}
            \policy_{\text{perf}}(\state)\qquad& \traj^{\tilde\policy}_{\dyn\big(\state,\policy_\text{perf}(\state\big)}(t) \text{ is safe and live}\\
            \tilde\policy(\state)&\text{otherwise}
        \end{cases}
    \end{equation}
    \item Reaching a safe stop or orbit.
\end{itemize}

==> figuresFinal/fig_lunar_lander_margins.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.8\columnwidth]{figuresFinal/lunar_lander/obstacle_and_target.png}
    \caption{Lunar lander target and safety margins depicted. The boundary of the constraint polygon is depicted in red. The boundary of the target set is depicted in green.}
    \label{fig:lunar_lander_margins}
\end{figure}
